Predicting Citywide Crowd Flows in Irregular Regions Using Multi-View Graph Convolutional Networks

Being able to predict the crowd flows in each and every part of a city, especially in irregular regions, is strategically important for traffic control, risk assessment, and public safety. However, it is very challenging because of interactions and spatial correlations between different regions. In addition, it is affected by many factors: i) multiple temporal correlations among different time intervals: closeness, period, trend; ii) complex external influential factors: weather, events; iii) meta features: time of the day, day of the week, and so on. In this paper, we formulate crowd flow forecasting in irregular regions as a spatio-temporal graph (STG) prediction problem in which each node represents a region with time-varying flows. By extending graph convolution to handle the spatial information, we propose using spatial graph convolution to build a multi-view graph convolutional network (MVGCN) for the crowd flow forecasting problem, where different views can capture different factors as mentioned above. We evaluate MVGCN using four real-world datasets (taxicabs and bikes) and extensive experimental results show that our approach outperforms the adaptations of state-of-the-art methods. And we have developed a crowd flow forecasting system for irregular regions that can now be used internally.

==> abstract.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}
Being able to predict the flow of crowds in each and every part of a city, especially in \textit{irregular regions}, is strategically important for traffic control, risk assessment, and public safety. However, it is a very challenging problem because of interactions and spatial correlations between different regions. In addition, it is affected by many factors: i) multiple \textit{temporal correlations} among different time intervals: closeness, period, trend; ii) complex \textit{external} influential factors: weather, events, \etc{}; iii) \textit{meta} features: time of the day, day of the week, and so on. 

In this paper, we formulate the crowd flow forecasting in irregular regions of a city as a \textit{spatio-temporal graph} (STG) prediction problem in which each node represents a region with the time-varying inflow/outflow of crowds. By extending the \textit{graph convolution} to handle the spatial information, we propose the \textit{spatial graph convolution}, and use it to build a \textit{multi-view graph convolutional network} (MVGCN) for the crowd flow forecasting problem, where different views can capture different factors mentioned above. We evaluate MVGCN using four real-world mobility datasets (taxicabs and bikes) and the extensive experimental results show that our approach outperforms the adaptations of state-of-the-art methods, like recurrent neural networks and Gaussian Markov random field based models. We have developed a real-time crowd flow forecasting system for irregular regions that can be used internally now, and will be available later in our previous UrbanFlow system. %\footnote{http://urbanflow.chinacloudsites.cn/}. 
% 
% Then, we propose a multi-view deep learning approach, to collectively forecast inflow/outflow in each and every node of an STG. 
% More specifically, 
% we present a \textit{\underline{S}patio-t\underline{E}mporal graph convolutional r\underline{E}sidual \underline{Net}work} (entitled SEENet), to collectively forecast inflow/outflow in each and every vertex of an STG. More specifically, we propose a \textit{Spatial graph Convolutional Residual} (SCR) unit to capture spatial correlations and interactions between different nodes, and integrate the geospatial position. Then we stack multiple SCRs (SCR-Net) to model more complex spatial patterns like multi-hop interactions. Moreover, we employ different SCR-Nets to model different temporal properties, including closeness, period (\eg{} daily and weekly), and trend (monthly, quarterly). We design a general fusion module to fuse data across different domains, including various types of external factors (like weather), meta data (\eg{} time of the day) as well as the outputs of all SCR-Nets based on two methods: gating mechanism and sum fusion. 
% Extensive experiments on four different taxicab/bike data demonstrate our \model{} outperforms 12 well-known methods based on three metrics. 
\end{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
	Multi-view learning, neural network, spatio-temporal prediction
\end{IEEEkeywords}
